Receptive-field-regularized CNN variants for acoustic scene classification

Acoustic scene classification and related tasks have been dominated by Convolutional Neural Networks (CNNs). Top-performing CNNs use mainly audio spectograms as input and borrow their architectural design primarily from computer vision. A recent study has shown that restricting the receptive field (RF) of CNNs in appropriate ways is crucial for their performance, robustness and generalization in audio tasks. One side effect of restricting the RF of CNNs is that more frequency information is lost. In this paper, we perform a systematic investigation of different RF configuration for various CNN architectures on the DCASE 2019 Task 1.A dataset. Second, we introduce Frequency Aware CNNs to compensate for the lack of frequency information caused by the restricted RF, and experimentally determine if and in what RF ranges they yield additional improvement. The result of these investigations are several well-performing submissions to different tasks in the DCASE 2019 Challenge.

==> sections/at.tex <==
%!TEX root = ../main.tex

\subsection{Baseline}

We trained a DenseNet DN1 (Section~\ref{sec_dn}) and different variants of RN1 (Section~\ref{sec_resnet}) on the curated data. The best performing ResNet-based model on our cross-validation was models with both Shake-Shake and the Frequency-Aware CNNs.

\subsection{Low Learning-rate Noisy Training}
To integrate the noisy data, we trained our models on the noisy labels but with a small learning rate that is $0.2$ of the learning rate used for training on the curated data.


\subsection{Adaptive-Weighting of Noisy Samples}\label{sec:adaptweight}
We calculate the \emph{inner product} of the noisy ground truth vector with the vector of the predicted probabilities from the noisy samples. 
We then average the resulting scalar while training each sample. 
The resulting average is then used to weight the loss of each noisy sample, when seen by the network in the future epochs. 
This will weight down the noisy samples, based on the ground truth and network predictions disagreement.

\subsection{Noisy Samples Selection}\label{sec:samplesel}
At a later stage, we average the weights of the noisy samples (as explained in the previous section) that resulted from different runs.
We use a threshold to select only samples with higher weights, to be used for training new models.

\subsection{Inverse-Lwlwrap Class Weighting}\label{sec:lwlrap}
We noticed that some classes are harder to learn, or have lower Lwlwrap scores. 
To tackle this issue, we use the inverse of the lwlwrap of a class, to weight the class's vector term in the cross-entropy loss function.

\subsection{Submissions}
We use the average of different combinations of the models trained with the aforementioned setups for our final submissions. The results on the Kaggle leader-board are provided in Table~2.



==> sections/task1a.tex <==
%!TEX root = ../main.tex
\textbf{Single model submission:}
Our first submission consists of the predictions of a single model trained on the whole development set with no validation set. We average the prediction of the model every 5 epochs, after epoch 300. The results on the Kaggle leader boards are provided in Table~2.
\\\textbf{Average over 4-fold cross-validation submission:}
We randomly split the development set into 4 folds regardless of the city or the scene id. We then train 4 models on these splits and submitted the average of the predictions of these models.
\\\textbf{Average different variants submissions:}
We trained different variants of DenseNet and ResNet (as explained in Section~\ref{sec:arcs}) and averaged different combinations of these models for our submissions 3 and 4 (16 models and 7 models respectively).


==> sections/task1b.tex <==
%!TEX root = ../main.tex
Task 1.B is to classify audio snippets into acoustic scene classes, where the model has to deal with the nuisance of a recording device mismatch between the training and the testing data.
A small set of parallel recordings are provided in the training to be used as adaptation data, however, the majority of the training data is from a single device which is not targeted in the challenge test set.
Hence, a model has to learn device-invariant representations such that the model can generalize on the new samples from various devices.

As studied in~\cite{eghbal2018deep}, CNNs have shown to suffer from significant performance degradation when dealing with mismatched distributions at inference time.
To tackle this issue, in our submission to Task 2.B we integrate a \emph{Two-Sample Test (TST)}
\footnote{Comparing samples from two probability distributions, by proposing statistical tests of the null hypothesis that these distributions are equal against the alternative hypothesis that these distributions are different~\cite{gretton2012kernel}.} based on kernel Maximum Mean Discrepancy (MMD)~\cite{gretton2012kernel} to encourage our model to learn device-invariant embeddings, such that the embedding distribution of various devices are indistinguishable from each other.

% Besides their theoretical Guarantees (Theorem 1 in~\cite{gretton2012kernel}),  one additional 
One advantage of TST frameworks compared to pair-wise matching techniques is that, as these methods are trying to match the distributions, they do not require paired recordings.
This provides more freedom in terms of mini-batch selection and data augmentation, as the model only needs two sets of (even unpaired) samples from two devices.

Another family of models capable of dealing with unpaired distribution matching are adversarial frameworks such as Generative Adversarial Networks (GANs)~\cite{goodfellow2014generative}.
One advantage of the TST frameworks over the adversarial ones is that TST frameworks do not require a parametric discriminator. Training a discriminator increases the complexity of the model, and introduces new problems to the training such as instability and mode collapse, which require additional efforts to solve~\cite{eghbal2019mixture}.

% However, one of the drawbacks of TST frameworks such as MMD, is that they require large batch-size for training to compute  meaningful statistics from the model's embeddings.
% This constrain is not ideal, since by increasing the batch-size, the memory requirements also rises which is inefficient.

% Authors in~\cite{li2017mmd} propose a TST framework that benefits from 

\subsubsection{The Proposed Domain Adaptation Objective}
% For the choice of MMD, we use an efficient implementation of permutation tests proposed in~\cite{sutherland2016generative}.
We begin with the definition of our \acro{mmd} measure between two sets of samples from two different distributions.
Let $k$ be the Gaussian \acro{rbf} kernel.
Then we use an estimation of $\mmd(P, Q)$ between two distributions $P$ and $Q$, given a set of $m$ samples $X = \{X_1, \dots, X_m \} \simiid P$ and a set of $m$ samples $Y = \{ Y_1, \dots, Y_m \} \simiid Q$,\footnote{We assume the number of samples from the two distributions are equal.} defined as:
\begin{equation}
\begin{split}
  \acro{mmd}(X, Y)  := &\frac{1}{m^2} \sum_{i \ne i'} k(X_i, X_{i'})  + \frac{1}{m^2} \sum_{j \ne j'} k(Y_j, Y_{j'})\\
  &-\frac{2}{m^2} \sum_{i \ne j} k(X_i, Y_j)
\label{eq:mmd-u}
\end{split}
\end{equation}
As explained in~\cite{gretton2012kernel}, $\mmd_k(P, Q) = 0$ if and only if $P = Q$.

We now define $\mathcal{F}_{l}(x)$ as the activations of a hidden layer $l$, in a feed-forward neural network $\mathcal{F}$, given an input spectrogram $x$.
Given the definitions above, our domain adaptation loss to learn device-invariant representations in layer $l$ is as follows:
\begin{equation}
\mathcal{L}_{\acro{mmd}} =  \acro{mmd}(\mathcal{F}_{l}(x_i^d)_{i=1}^{m}, \mathcal{F}_{l}(x_j^{d'})_{j=1}^{m})
\end{equation}
where $x_i^d$ and $x_j^{d'}$ are two spectrograms of audio snippets from devices $d$ and $d'$, respectively.
Please note that  $x_i^d$ and $x_j^{d'}$ are not required to be parallel recordings of the same scene, hence are sampled randomly in every minibatch.

For classification, we use Categorical Cross
Entropy (CCE) loss, which is combined with our domain adaptation loss as follows:
\begin{equation}
\mathcal{L}_{\acro{hyb}} =  \mathcal{L}_{\acro{mmd}} + \mathcal{L}_{\acro{CCE}} 
\end{equation}
where $\mathcal{L}_{\acro{hyb}}$ is our hybrid loss, and $\mathcal{L}_{\acro{CCE}}$ is the categorical cross entropy loss used for classification.

\subsubsection{Training setup}
Our training consists of two steps: 1) the classification step, and 2) the hybrid step.
In the classification step, we train our model for a full epoch with the CCE loss, using a randomly selected mini-batch of size 10 from the full training set.
Each mini-batch is augmented with \textit{mix-up}~\cite{zhangMixupEmpiricalRisk2017}.
% 
In the hybrid step, our model is trained using the hybrid loss, on a randomly-selected set of parallel samples\footnote{Samples from the training set that have recordings in all A, B and C devices.}.
First, two devices are randomly chosen out of the 3 available devices, then a number of 10 samples from each selected device is randomly selected to create a 20-samples mini-batch.
This mini-batch is further augmented via \textit{mix-up}.
Our model is trained iteratively using the classification and the hybrid steps.
\\\\\textbf{Architectures}:
We use two receptive-field-regularized CNN architectures from~\cite{Koutini2019Receptive}, namely Resnet and Shake-Shake~\cite{gastaldi2017shake}. 
We use RN1 (Section~\ref{sec_resnet}) with Shake-Shake and our proposed Frequency-Aware CNN layers.
The exact architecture of our ResNet is provided in Table~\ref{tab_resnet_configs}, but with half the number of channels.
% 
% In each residual block, two parallel convolutional blocks are first combined with a random weight (both in forward and backward pass), and further added to the residual connection.
% We use the same ResNet architecture as we described, but only add the Shake-Shake regularization.
We use a 4-fold Cross-Validation (CV), and use the average prediction of the resulting 4 models in our final prediction.
Additionally, we use snap-shot averaging as explained above.

\subsubsection{Results}
\label{sec:task1b:results}

In the following, we detail our 4 submissions to the DCASE'19 Task 1.B. The results on the Kaggle leader-boards are provided in Table~2.
\\\textbf{1) Shake-Shake/ResNet with Snapshot averaging:} In this submission, we use our ResNet and  Shake-Shake model. From each architecture, 4 models are trained using our 4 folds CV. The predictions from models of all the 4 folds are averaged for each test file.
Additionally, we use the average prediction of 20 snapshots from each model as explained above for our final prediction.
\\\textbf{2) Shake-Shake/ResNet:} Similar to our first submission, this submission uses an average prediction of our ResNet and Shake-Shake architectures. Instead of snap-shot averaging, only the best model from each fold was used in the final prediction averaging.
\\\textbf{3) Shake-Shake with Snapshot averaging:} This submission is similar to our first submission, but only Shake-Shake model is used.
\\\textbf{4) Shake-Shake:} In this submission, a similar approach to our second submission is used, but only using our Shake-Shake model.




% \begin{figure}[h]
%   \centering
%   \centerline{\includegraphics[width=.5\columnwidth]{img/t1b_f1_loss.png}
%     \includegraphics[width=.5\columnwidth]{img/t1b_f1_acc.png}}
%   \caption{The $\mathcal{L}_{\acro{hyb}}$ and $\mathcal{L}_{\acro{CCE}}$ on the training set (top), and per-device accuracies on the test set (CV fold 1).}
%   \label{fig:results_t1b}
% \end{figure}

\begin{table}[ht!]
\centering
\begin{tabular}{ @{}lccc@{} }
\toprule
  &SID& Kag. Pub&Kag. Prv.\\
\midrule
Task 1.A&&& \\
Single Res Snp& 1& 82.83& 81.33\\
CV Res Snp& 2& 83.50& 83.00 \\
CV Res-FACNN Snp& -&80.66 & 83.66 \\
Preact\textbackslash Res-FACNN Snp & 3 & 80.50 & 82.50 \\
Preact\textbackslash Res-FACNN\textbackslash Dense Snp & 4 & 82.00 & 82.83 \\
\hline
Task 1.B&&&\\
CV Res\textbackslash Shake-FACNN Snp& 1& 75.00& 77.50\\
CV Res\textbackslash Shake-FACNN& 2&74.33 &  76.83   \\
CV Shake-FACNN Snp                 & 3& 75.66& 75.16 \\
CV Shake-FACNN & 4& 74.33& 75.83 \\ 
CV Shake-FACNN (no DA)  & -& 73.66& 73.00 \\ 
\hline
Task 2&&&\\
Average 1& 1& .728& - \\
Average 2& 2& .725& -  \\
CV Shake-FACNN& -& .715 & -  \\
\bottomrule
\end{tabular}
\label{tab:all_results}
\caption{The accuracy of different methods on various test sets. Snp: Snapshot averaging, Shake: Shake-Shake ResNet, Res: ResNet. DA: Domain Adaptation. The details of the submissions are explained in their respective sections with their corresponding Submission Ids (SID). }
\end{table}

